Fingerprinting of Machines in Critical Systems for Integrity Monitoring and Verification

As cyber threats continue to evolve and diversify, it has become increasingly challenging to identify the root causes of security breaches that occur between periodic security assessments. This paper explores the fundamental importance of system fingerprinting as a proactive and effective approach to addressing this issue. By capturing a comprehensive host's fingerprint, including hardware-related details, file hashes, and kernel-level information, during periods of system cleanliness, a historical record is established. This historical record provides valuable insights into system changes and assists in understanding the factors contributing to a security breach. We develop a tool to capture and store these fingerprints securely, leveraging the advanced security features. Our approach presents a robust solution to address the constantly evolving cyber threat landscape, thereby safeguarding the integrity and security of critical systems.

==> Hashes.tex <==
% Hashing functions are critical in computer security, transforming input data into fixed-length hashes. The irreversible nature of hashing ensures the security of the original input. Hash functions primarily serve to maintain data integrity. By comparing the original data's hash with the stored hash, any discrepancies indicate potential tampering.
% % \begin{figure*}
% % \centering
% % \includegraphics[scale=.5]{Full version/hash.png}
% %   \caption{Construction of hash}
% % \end{figure*}
% Hash functions efficiently map inputs of varying lengths to fixed-length outputs, facilitating consistent hash comparisons. However, the occurrence of collisions, where different inputs yield identical hashes, poses a significant challenge. This awareness has prompted the creation of algorithms aimed at minimizing such risks.
% Key attributes of hash functions include pre-image resistance, second pre-image resistance, and collision resistance. Pre-image resistance prevents the derivation of the original input from its hash, enhancing security against reverse engineering. Second pre-image resistance and collision resistance safeguard against finding alternative inputs that produce the same hash.

% In file integrity verification, cryptographic hash functions are essential for detecting unauthorized or accidental file modifications. Regular file hash comparisons can quickly indicate any changes, intentional or unintentional. Legacy algorithms such as MD4 and MD5 are considered insecure due to vulnerabilities to collision attacks, making them unreliable for integrity verification. Likewise, SHA-1 is also discouraged due to analogous security flaws. Currently, SHA-2, particularly SHA-256, is esteemed in scholarly discourse as a robust cryptographic option, demonstrating formidable resistance to collision attacks.

% In addition to their role in the verification of system integrity, we further explore the importance of hash functions in safeguarding directories within operating systems. We present two distinct tables—one related to Linux (Table I) and the other pertaining to Windows (Table II)—that enumerate critical system directories. These directories are consistently monitored for unauthorized alterations or tampering. By creating and periodically comparing the hash values of files contained within these directories, system administrators can detect potential security breaches or integrity violations. This approach highlights the practical application of hash functions in reinforcing the security infrastructure of both Linux and Windows operating systems.


Hash functions constitute a cornerstone of computer security, converting inputs of variable lengths into outputs of fixed lengths. Cryptographic hash functions, such as SHA-256, are esteemed for their exceptional resilience against collision and pre-image attacks. These characteristics render SHA-256 a formidable option for the verification of data integrity and the identification of unauthorized alterations.

In the domain of file integrity verification, SHA-256 assumes a pivotal role by producing hashes for essential files, thus enabling system administrators to detect tampering through systematic hash comparisons. Its utilization in system security encompasses the oversight of critical directories within both Linux and Windows operating systems. Through the process of hashing and the regular comparison of directory contents, SHA-256 guarantees the identification of unauthorized modifications, thereby bolstering the overarching security architecture.

We have systematically delineated the essential directories and files for which hash monitoring is being conducted. Tables I and II provide a comprehensive enumeration of the critical files and directories pertinent to Windows-Based Systems and Linux-Based Systems, respectively.



==> Linux.tex <==
% Linux details go here

% \subsection{List Installed Packages}
% In order to compile a list of installed packages on a Linux system and subsequently generate hash values for integrity verification, the following procedures are recommended:

% \begin{enumerate}

% \item For Debian-based systems, such as Ubuntu, the 'dpkg' command proves invaluable for cataloging all installed packages.
% % The command to achieve this is as follows:

% \item Conversely, Red Hat-based systems like CentOS and Fedora employ the 'rpm' command for similar purposes. 

% \end{enumerate}


Documenting every installed package on a Linux system is crucial for a number of reasons, including security and system upkeep. Several Linux distributions have dedicated commands to export an exhaustive list of installed packages in order to accomplish this. For example, the \textit{rpm} command used with \textit{rpm -qav -info} on Red Hat-based systems, such Fedora and CentOS, enables users to create a comprehensive list. On Debian-based systems, such as Ubuntu, the equivalent commands \textit{apt list -installed} and \textit{dpkg -list} accomplish the same thing. These commands provide users with flexibility according to their preferred Linux distribution by making it easier to generate an extensive catalogue of installed packages.

System administrators and security experts can monitor software installations, software installation dates, and evaluate the integrity of the system with the help of the resulting lists, which are useful benchmarks for verifying unauthorised changes. These lists can also be used for vulnerability assessments and security audits, which helps to maintain the Linux system's trusted status. Accurate documentation of installed packages is essential for research and system maintenance in order to preserve system security, stability, and adherence to organisational norms.


% Protecting virtual machines is a major concern when it comes to Linux security, and this is achieved by preserving their '.vmx' files, which are similar to Windows' Virtual Machine Configuration Files. In Linux virtualization setups, these '.vmx' files are crucial, acting as the foundation for defining and managing basic settings for every virtual machine. Like their Windows counterparts, they contain critical data on network adapters, CPU usage, system settings, and other important aspects. Beyond just hardware specs, '.vmx' files also contain vital information about the guest operating system, virtual devices (such CD/DVD drives and '.vmdk' files), power management settings, customizations, and snapshots. This comprehensive data repository renders '.vmx' files indispensable for effectively configuring, managing, and securing the characteristics and performance of virtual machines in Linux environments. Because of this extensive data store, '.vmx' files become essential for efficiently setting up, controlling, and safeguarding the features and functionality of virtual machines running Linux.

\begin{figure*}
%\raggedright
\centering
\includegraphics[scale=.4]{Full version/Arch.drawio.png}
  \caption{Proposed Steps to capture fingerprint  }
\end{figure*}


% In Linux the ’.vmx’ files serve as a cornerstone for protecting the integrity and confidentiality of virtual machine configurations, playing a pivotal role in ensuring that virtualized environments are resilient against
% potential threats and vulnerabilities. With a clear understanding of the significance of these files, system  administrators. In Linux security, the '.vmx' files serve as a cornerstone for protecting the integrity and confidentiality of virtual machine configurations, playing a pivotal role in ensuring that virtualized environments are resilient against potential threats and vulnerabilities. With a clear understanding of the significance of these files, system administrators, security experts, and Linux users can take proactive measures to safeguard these critical assets and maintain the overall security posture of their virtualized infrastructure.

==> Windows.tex <==
Security threats in the Windows OS are significant. The Windows OS utilizes an internet security suite comprising antivirus, firewall, and anti-spyware for its defense. Nevertheless, it is not without flaws. Users with admin rights may inadvertently install internet applications, facilitating malware entry without alerting security systems. Conventional security mechanisms, such as antivirus software, are dependent on known signatures, thereby exposing users to zero-day threats. Physical interference with disk storage poses a substantial risk, as attackers can manipulate data or deploy keyloggers to extract sensitive information. These issues highlight the necessity for comprehensive security strategies within the Windows OS landscape. Herein, system fingerprinting is pertinent. In the realm of Windows security, fingerprinting encompasses a multifaceted strategy for system examination and safeguarding. This extensive process comprises several essential tasks. Initially, a comprehensive inventory of all installed software and packages on the operating system is compiled using various Windows commands. This process entails accessing registry keys and subkeys, notably the primary root keys, including HKEY LOCAL MACHINE and HKEY USERS, to extract information on software packages, such as their versions and installation paths.

To enhance the system fingerprinting process within a Windows environment, it is crucial to safeguard essential registry data. The Windows registry acts as a centralized archive for system configurations, user preferences, and installed software details, making it vital for monitoring system changes. Recording important registry entries, especially from HKEY LOCAL MACHINE and HKEY CURRENT USER, aids in tracking critical system information such as startup applications, network configurations, and other security settings. By routinely backing up this registry data, security analysts can identify unauthorized changes, thus creating a thorough timeline of system modifications. This practice is vital for threat mitigation, as cyber adversaries often alter registry keys to maintain access to compromised systems or to disable security measures.

The acquisition of system information is facilitated by commands such as \textit{wmic bios get Manufacturer, Name, Version, SerialNumber} and \textit{Get-WmiObject -Class Win32{\_}BIOS}, which provide comprehensive BIOS data. Additionally, \textit{Get-WmiObject -Class Win32{\_}OperatingSystem | Select-Object Caption, Version, InstallDate} offers crucial details regarding the Windows operating system, while other commands furnish information on PCIE slots, network adaptors, and sound cards. Thus, the documentation of hardware configurations ensures effective monitoring of changes in system settings. The preservation of system configuration and hardware data is essential for system fingerprinting, as it establishes a reference point for identifying unauthorized modifications. Hardware alterations may be exploited by malicious entities, or the changes themselves may originate from malicious actions. The maintenance of such records is instrumental in recognizing anomalies and potential security risks, thereby enabling prompt corrective measures to safeguard system integrity.


